Orbits of very distant asteroid satellites

The very wide binary asteroid (VWBA) population is a small subset of the population of known binary and multiple asteroids made of systems with very widely orbiting satellites and long orbital periods, on the order of tens to hundreds of days. The origin of these systems is debatable, and most members of this population are poorly characterized. We have compiled all available high-angular resolution imaging archival data of VWBA systems from large ground- and space-based telescopes. We measure the astrometric positions of the satellite relative to the primary and analyze the dynamics of the satellites using the Genoid genetic algorithm. Additionally, we use a NEATM thermal model to estimate the diameters of two systems, and we model the orbit of Litva's inner satellite using photometric lightcurve observations. We determine the effective diameters of binary systems Christophedumas and Alconrad to be 4.7 + 0.4km and 5.2 + 0.3km respectively. We determine new orbital solutions for five systems, Huenna, Litva, (3548) Eurybates, Pauling, and Alconrad. We find a significantly eccentric best-fit orbital solution for the outer satellite of Litva, a moderately eccentric solution for Alconrad, and a nearly circular solution for Pauling. We also confirm previously reported orbital solutions for (379) Huenna and Eurybates. It is unlikely that BYORP expansion could be solely responsible for the formation of VWBAs. It is possible that the satellites of these systems were formed through YORP spin-up and then later scattered onto very wide orbits. Additionally, we find that some members of the population are unlikely to have formed satellites through YORP spin-up, and a collisional formation history is favored. In particular, this applies to VWBAs within large dynamical families, or large VWBA systems such as Huenna and NASA's Lucy mission target Eurybates.

==> Makefile <==
all:
	-make latex
	-make biblio
	-make latex
	-make pdf

latex:
	pdflatex "\def\destination{arxiv} \input{main.tex}"
	#pdflatex "\def\destination{aanda} \input{main.tex}"

bib:
	bibtex main

pdf:
	mv main.pdf 2023-Article-TITLE.pdf

clean:
	rm -f *.bbl *.aux *.nav *.out *.dep *d.vi *.snm *.toc *.blg *.log *~ *.abs

src:
	tar cvzf TITLE-Sources.tar.gz main.tex *cls *sty Makefile gfx aux data frontback scripts


==> aux/macros.tex <==
% Author comment
\newcommand{\KM}[1]{\textcolor{cyan}{[#1]}}
\newcommand{\BC}[1]{\textcolor{orange}{[#1]}}
%
% Edition
\renewcommand{\sup}[1]{\ensuremath{^{\textrm{#1}}}}
\newcommand{\sub}[1]{\ensuremath{_{\textrm{#1}}}}
\newcommand{\src}{\sup{\textcolor{blue}{[Citation needed]}}}
%


==> frontback/abstract.tex <==
abstract


==> frontback/abstract_aa.tex <==
\abstract
  % context heading (optional)
   {\textbf{CHECK if not co-author forgotten!!}}
   % aims heading (mandatory)
   {}
  % methods heading (mandatory)
   {}
  % results heading (mandatory)
   {}
  % conclusions heading (optional), leave it empty if necessary 
   {}



==> frontback/abstract_aa_trash.tex <==
\abstract
  % context heading (optional)
   {The very wide binary asteroid (VWBA) population is a small
   subset of the population of known binary and multiple asteroids
   made of  %containing
   systems 
   % \BC{characterized by orbital periods over 50\,days.}
   with very widely orbiting satellites and long orbital periods, on the order of tens to hundreds of days. 
   The origin of these systems is debated, and 
   most %the
   members of this population are poorly characterized.}
   % aims heading (mandatory)
   {We aim to develop orbital solutions for some members of the VWBA population, allowing us to constrain possible formation pathways for this unique population.}
  % methods heading (mandatory)
   {We have compiled all available high-angular resolution imaging
   archival data of VWBA systems from large ground- and space-based 
   telescopes. %in order
   We measure the astrometric positions of the satellite relative to the 
   primary at each epoch and analyze the dynamics of the satellites using the \genoid 
   genetic algorithm. Additionally, we use a NEATM thermal model to estimate the diameters of two systems, and we model the orbit of Litva's inner satellite using photometric lightcurve observations. }
  % results heading (mandatory)
   {We determine the effective diameters of binary systems (17246) Christophedumas and (22899) Alconrad to be $4.7\pm0.4$km and $5.2\pm0.3$ km respectively. We determine new orbital solutions for five systems, (379) Huenna, (2577) Litva, (4674) Pauling, (17246) Christophedumas and (22899) Alconrad.
   We find a significantly eccentric ($e=0.30$)
   best-fit orbital solution for the outer satellite of (2577) Litva, moderately eccentric ($e=0.13$)
   solutions for (22899) Alconrad,
   and a nearly circular solution for (4674) Pauling ($e=0.04$).
   We also confirm the orbital solution for (379) Huenna 
   reported by \citet{2022Icar..38215013V} with the addition of new observations.}
  % conclusions heading (optional), leave it empty if necessary 
   {It is unlikely that BYORP expansion could be solely responsible for the
   formation of VWBAs, as only (4674) Pauling matches the necessary
   requirements for active BYORP expansion.
   It is possible that the satellites of these systems were formed
   through YORP spin-up and then later scattered onto very wide orbits.
   Additionally, we find that some members of the population are unlikely
   to have formed satellites through YORP spin-up,
   and a collisional formation history is favored.
   % \BC{This particularly applies to VWBAs within dynamical families,
   % such as (22899) Alconrad, (17246) Christophedumas, or the large (379)
   % Huenna, akin to (3548) Eurybates, target of the NASA Lucy mission.}}
   %\BC{Consider mentioning Lucy/Eurybates in the abstract for visibility}}
   In particular, this applies to VWBAs within large dynamical families,
   such as (22899) Alconrad and (2577) Litva, or large VWBA systems such as (379) Huenna and Lucy mission target (3548) Eurybates.}



==> frontback/ack.tex <==
acknowloedge

